Detecting Spells in Fantasy Literature with a Transformer Based Artificial Intelligence

Transformer architectures and models have made significant progress in language-based tasks. In this area, is BERT one of the most widely used and freely available transformer architecture. In our work, we use BERT for context-based phrase recognition of magic spells in the Harry Potter novel series. Spells are a common part of active magic in fantasy novels. Typically, spells are used in a specific context to achieve a supernatural effect. A series of investigations were conducted to see if a Transformer architecture could recognize such phrases based on their context in the Harry Potter saga. For our studies a pre-trained BERT model was used and fine-tuned utilising different datasets and training methods to identify the searched context. By considering different approaches for sequence classification as well as token classification, it is shown that the context of spells can be recognised. According to our investigations, the examined sequence length for fine-tuning and validation of the model plays a significant role in context recognition. Based on this, we have investigated whether spells have overarching properties that allow a transfer of the neural network models to other fantasy universes as well. The application of our model showed promising results and is worth to be deepened in subsequent studies.

==> tables/cross_universe_comparison.tex <==

\begin{table}[t] 
\begin{small}
    \begin{tabular}{ c l || l | l | l}
        & Einträge & \textbf{Sentence-Split} & \textbf{Paragraph-Split} & \textbf{Sequence-Split} \\
        \toprule
         \multirow{3}{*}{\rotatebox[origin=tr]{90}{\parbox{1.7cm}{\centering{Eragon}}}} 
         & \textbf{Alle } & 14.009 & 4.061 & 619 \\
         & \textbf{Positive} & 65 & 32 & 1 \\
         & \textbf{True Positive} & 24 & 18 & 0 \\
        \hline
         \multirow{3}{*}{\rotatebox[origin=tr]{90}{\parbox{1.7cm}{\centering{The Fareway Paladin}}}} 
         & \textbf{Alle } & 6.155 & 2.434 & 262 \\
         & \textbf{Positive} & 67 & 20 & 5 \\
         & \textbf{True Positive} & 25 & 18 & 2 \\
    \end{tabular}
\end{small}
\caption{Ergebnisse der Untersuchungen von Fremduniversen} 
\label{tab:study_cross_overview}
\end{table}

==> tables/metric_sequence_1a.tex <==
\begin{table}[t]
\begin{subtable}{0.48\textwidth}
    \begin{small}
        \begin{tabular}{ c l | l l}
            \multicolumn{2}{l}{} & \multicolumn{2}{c}{Predicted} \\
            &  & \textbf{Positive} & \textbf{Negative} \\
        \cline{2-4}
            \multirow{2}{*}{\rotatebox[origin=tr]{90}{True}} & \textbf{Positive} & 279 TP & 5 FN \\
        & \textbf{Negative} & 78 FP & 13880 TN \\[5pt]
        & \multicolumn{3}{l}{ F1-Sore: 0,8705} \\
        \end{tabular} 
    \end{small}
    \caption{Big Dataset} 
\label{tab:study_sentence_combined}
\end{subtable}
\hspace*{0.02\textwidth} 
\begin{subtable}{0.48\textwidth}
    \begin{small}
        \begin{tabular}{ c l | l l}
            \multicolumn{2}{l}{} & \multicolumn{2}{c}{Predicted}  \\
            &  & \textbf{Positive} & \textbf{Negative} \\
        \cline{2-4}
             \multirow{2}{*}{\rotatebox[origin=tr]{90}{True}} & \textbf{Positive} & 112 TP & 0 FN \\
            & \textbf{Negative} & 67 FP & 14.063 TN \\[5pt]
            & \multicolumn{3}{l}{F1-Sore: 0,7698} \\
        \end{tabular} 
    \end{small}
    \caption{Incantation Dataset} 
    \label{tab:study_sentence_incantations}
\end{subtable}
\caption{Metric of trainend model 1a}
\label{tab:study_sentence_split}
\end{table}

==> tables/metric_sequence_1b.tex <==
\begin{table}[t]
\begin{subtable}{0.48\textwidth}
    \begin{small}
        \begin{tabular}{ c l | l l}
            \multicolumn{2}{l}{} & \multicolumn{2}{c}{Predicted} \\
            &  & \textbf{Positive} & \textbf{Negative} \\
        \cline{2-4}
            \multirow{2}{*}{\rotatebox[origin=tr]{90}{True}} & \textbf{Positive} & 278 TP & 6 FN \\
            & \textbf{Negative} & 75 FP & 13.883 TN \\[5pt]
            & \multicolumn{3}{l}{F1-Sore: 0,8728} \\
        \end{tabular} 
    \end{small}
    \caption{Big Dataset} 
\label{tab:study_sentence_tokenizer_combined}
\end{subtable}
\hspace*{0.02\textwidth} 
\begin{subtable}{0.48\textwidth}
    \begin{small}
        \begin{tabular}{ c l | l l}
            \multicolumn{2}{l}{} & \multicolumn{2}{c}{Predicted}  \\
            &  & \textbf{Positive} & \textbf{Negative} \\
        \cline{2-4}
            \multirow{2}{*}{\rotatebox[origin=tr]{90}{True}} & \textbf{Positive} & 111 TP & 1 FN \\
            & \textbf{Negative} & 42 FP & 14.088 TN \\[5pt]
            & \multicolumn{3}{l}{F1-Sore: 0,8377} \\
        \end{tabular} 
    \end{small}
    \caption{Incantation Dataset} 
    \label{tab:study_sentence_tokenizer_incantations}
\end{subtable}
\caption{Metric of trainend model 1b}
\label{tab:study_sentence_tokenizer_split}
\end{table}

==> tables/metric_sequence_2.tex <==
\begin{table}[t]
\begin{subtable}{0.48\textwidth}
    \begin{small}
        \begin{tabular}{ c l | l l}
            \multicolumn{2}{l}{} & \multicolumn{2}{c}{Predicted} \\
            &  & \textbf{Positive} & \textbf{Negative} \\
        \cline{2-4}
        \multirow{2}{*}{\rotatebox[origin=tr]{90}{True}} & \textbf{Positive} & 262 TP & 9 FN \\
        & \textbf{Negative} & 43 FP & 6.597 TN \\[5pt]
        & \multicolumn{3}{l}{F1-Sore: 0,9097} \\
        \end{tabular} 
    \end{small}
    \caption{Big Dataset} 
\label{tab:study_paragraph_combined}
\end{subtable}
\hspace*{0.02\textwidth} 
\begin{subtable}{0.48\textwidth}
    \begin{small}
        \begin{tabular}{ c l | l l}
            \multicolumn{2}{l}{} & \multicolumn{2}{c}{Predicted}  \\
            &  & \textbf{Positive} & \textbf{Negative} \\
        \cline{2-4}
            \multirow{2}{*}{\rotatebox[origin=tr]{90}{True}} & \textbf{Positive} & 106 TP & 2 FN \\
            & \textbf{Negative} & 23 FP & 6.780 TN \\[5pt]
            & \multicolumn{3}{l}{F1-Sore: 0,8945} \\
        \end{tabular} 
    \end{small}
    \caption{Incantation Dataset} 
    \label{tab:study_paragraph_incantations}
\end{subtable}
\caption{Metric of trainend model 2}
\label{tab:study_paragraph_split}
\end{table}

==> tables/metric_sequence_3a.tex <==
\begin{table}[t]
\begin{subtable}{0.48\textwidth}
    \begin{small}
        \begin{tabular}{ c l | l l}
            \multicolumn{2}{l}{} & \multicolumn{2}{c}{Predicted} \\
            &  & \textbf{Positive} & \textbf{Negative} \\
        \cline{2-4}
        \multirow{2}{*}{\rotatebox[origin=tr]{90}{True}} & \textbf{Positive} & 197 TP & 7 FN \\
        & \textbf{Negative} & 11 FP & 587 TN \\[5pt]
        & \multicolumn{3}{l}{F1-Sore: 0,9563} \\
        \end{tabular} 
    \end{small}
    \caption{Big Dataset} 
\label{tab:study_sequence_combined}
\end{subtable}
\hspace*{0.02\textwidth} 
\begin{subtable}{0.48\textwidth}
    \begin{small}
        \begin{tabular}{ c l | l l}
            \multicolumn{2}{l}{} & \multicolumn{2}{c}{Predicted}  \\
            &  & \textbf{Positive} & \textbf{Negative} \\
        \cline{2-4}
        \multirow{2}{*}{\rotatebox[origin=tr]{90}{True}} & \textbf{Positive} & 77 TP & 7 FN \\
        & \textbf{Negative} & 5 FP & 716 TN \\[5pt]
        & \multicolumn{3}{l}{F1-Sore: 0,9277} \\
        \end{tabular} 
    \end{small}
    \caption{Incantation Dataset} 
    \label{tab:study_sequence_incantations}
\end{subtable}
\caption{Metric of trainend model 3a}
\label{tab:study_sequence_split}
\end{table}

==> tables/metric_sequence_3b.tex <==
\begin{table}[t]
\begin{subtable}{0.48\textwidth}
    \begin{small}
        \begin{tabular}{ c l | l l}
            \multicolumn{2}{l}{} & \multicolumn{2}{c}{Predicted} \\
            &  & \textbf{Positive} & \textbf{Negative} \\
        \cline{2-4}
        \multirow{2}{*}{\rotatebox[origin=tr]{90}{True}} & \textbf{Positive} & 195 TP & 9 FN \\
        & \textbf{Negative} & 9 FP & 589 TN \\[5pt]
        & \multicolumn{3}{l}{F1-Sore: 0,9559} \\
        \end{tabular} 
    \end{small}
    \caption{Big Dataset} 
\label{tab:study_sequence_tokenizer_combined}
\end{subtable}
\hspace*{0.02\textwidth} 
\begin{subtable}{0.48\textwidth}
    \begin{small}
        \begin{tabular}{ c l | l l}
            \multicolumn{2}{l}{} & \multicolumn{2}{c}{Predicted}  \\
            &  & \textbf{Positive} & \textbf{Negative} \\
        \cline{2-4}
        \multirow{2}{*}{\rotatebox[origin=tr]{90}{True}} & \textbf{Positive} & 80 TP & 3 FN \\
        & \textbf{Negative} & 2 FP & 717 TN \\[5pt]
        & \multicolumn{3}{l}{F1-Sore: 0,9697} \\
        \end{tabular} 
    \end{small}
    \caption{Incantation Dataset} 
    \label{tab:study_sequence_tokenizer_incantations}
\end{subtable}
\caption{Metric of trainend model 3b}
\label{tab:study_sequence_tokenizer_split}
\end{table}

==> tables/metric_token_1a.tex <==
\begin{table}[t]
\begin{subtable}{0.48\textwidth}
    \begin{small}
        \begin{tabular}{ c l | l l}
            \multicolumn{2}{l}{} & \multicolumn{2}{c}{Predicted} \\
            &  & \textbf{Positive} & \textbf{Negative} \\
        \cline{2-4}
        \multirow{2}{*}{\rotatebox[origin=tr]{90}{True}} & 
        \textbf{Positive} & 274 TP & 10 FN \\
        & \textbf{Negative} & 129 FP & 13.829 TN \\[5pt]
        & \multicolumn{3}{l}{F1-Sore: 0,7977} \\
        \end{tabular} 
    \end{small}
    \caption{Big Dataset} 
\label{tab:study_token_combined}
\end{subtable}
\hspace*{0.02\textwidth} 
\begin{subtable}{0.48\textwidth}
    \begin{small}
        \begin{tabular}{ c l | l l}
            \multicolumn{2}{l}{} & \multicolumn{2}{c}{Predicted}  \\
            &  & \textbf{Positive} & \textbf{Negative} \\
        \cline{2-4}
            \multirow{2}{*}{\rotatebox[origin=tr]{90}{True}} & 
            \textbf{Positive} & 110 TP & 2 FN \\
            & \textbf{Negative} & 103 FP & 14.027 TN \\[5pt]
            & \multicolumn{3}{l}{F1-Sore: 0,6769} \\
        \end{tabular} 
    \end{small}
    \caption{Incantation Dataset} 
    \label{tab:study_token_incantations}
\end{subtable}
\caption{Metric of trainend model 1a}
\label{tab:study_token_split}
\end{table}

==> tables/metric_token_1b.tex <==
\begin{table}[t]
\begin{subtable}{0.48\textwidth}
    \begin{small}
        \begin{tabular}{ c l | l l}
            \multicolumn{2}{l}{} & \multicolumn{2}{c}{Predicted} \\
            &  & \textbf{Positive} & \textbf{Negative} \\
        \cline{2-4}
        \multirow{2}{*}{\rotatebox[origin=tr]{90}{True}} & 
        \textbf{Positive} & 54 TP & 230 FN \\
        & \textbf{Negative} & 57 FP & 13.901 TN \\[5pt]
        & \multicolumn{3}{l}{F1-Sore: 0,2880} \\
        \end{tabular} 
    \end{small}
    \caption{Big Dataset} 
\label{tab:study_token_tokenizer_combined}
\end{subtable}
\hspace*{0.02\textwidth} 
\begin{subtable}{0.48\textwidth}
    \begin{small}
        \begin{tabular}{ c l | l l}
            \multicolumn{2}{l}{} & \multicolumn{2}{c}{Predicted}  \\
            &  & \textbf{Positive} & \textbf{Negative} \\
        \cline{2-4}
            \multirow{2}{*}{\rotatebox[origin=tr]{90}{True}} & 
            \textbf{Positive} & 28 TP & 84 FN \\
            & \textbf{Negative} & 43 FP & 14.087 TN \\[5pt]
            & \multicolumn{3}{l}{F1-Sore: 0,3060} \\
        \end{tabular} 
    \end{small}
    \caption{Incantation Dataset} 
    \label{tab:study_token_tokenizer_incantations}
\end{subtable}
\caption{Metric of trainend model 1b}
\label{tab:study_token_tokenizer_split}
\end{table}

==> tables/overview_sequence_models.tex <==
\begin{table}[ht]
\begin{subtable}{\textwidth}
    \begin{tabular}{ c | l | l }
        & \multicolumn{2}{c}{\textbf{F1-Score}} \\
        # & Kombi & Inc  \\
        \cline{2-5}
        (1 a) & 0,8705 & 0,7698 \\
        (1 b) & 0,8728 & 0,8377 \\
        (2)   & 0,9097 & 0,8945 \\
        (3 a) & 0,9563 & 0,9277 \\
        (3 b) & 0,9559 & 0,9697 \\
    \end{tabular}
    \caption{Models based on sequence classification} 
\end{subtable}

\caption{Comparative overview of all sequence classification studies}{
The table shows an overview of the trained models for sequence classification with the corresponding F1 metrics.}
\label{tab:study_sequence_overview}
\end{table}

==> tables/overview_token_classification.tex <==
\begin{table}[ht]
\begin{subtable}{\textwidth}
    \begin{tabular}{ c | l | l }
        & \multicolumn{2}{c}{\textbf{F1-Score}} \\
        # & Full & Inc  \\
        \cline{1-3}
        (1 a) & 0,7977 & 0,6769 \\
        (1 b) & 0,2880 & 0,3060 \\
    \end{tabular}
    \caption{Models based on token classification} 
\end{subtable}

\caption{Comparative overview of all token classification studies}{
The table shows an overview of the trained models for token classification with the corresponding F1 metrics.}
\label{tab:study_token_overview}
\end{table}

==> tables/split_approaches.tex <==

\begin{table}[ht]
%\hspace*{-0.04\textwidth}    
\begin{small}
\begin{tabular}{ c l || l | l || l | l || l | l}
    \multicolumn{2}{l}{} & \multicolumn{2}{c}{Sentence-Split} & \multicolumn{2}{c}{Paragraph-Split} & \multicolumn{2}{c}{Sequence-Split} \\
    &   & \textbf{Train} & \textbf{Eval} & \textbf{Train} & \textbf{Eval} & \textbf{Train} & \textbf{Eval} \\
    \toprule
      & \textbf{Alle Einträge} & 64.355 & 14.242 & 31.324 & 6.911 & 3.640 & 805 \\
    \hline
    \hline
    \multirow{3}{*}{\rotatebox[origin=tr]{90}{\parbox{1.7cm}{\centering{Positive Einträge}}}}
    & \textbf{Nur Incantations} & 283 & 112 & 262 & 108 & 195 & 84 \\
    & \textbf{Kombiniert} & 773 & 284 & 721 & 271 & 541 & 204 \\
\end{tabular}
\end{small}
\caption{Size comparison of differently generated data sets}{ \begin{small}
A Trianings (Train) and an Evaluations (Eval) dataset are created by three different splits of the Harry Potter corpus. The table shows the number of all entries of the datasets created in this way. \end{small}} 
\label{tab:split_overview}
\end{table}
